Reinforcement Learning with Function-Valued Action Spaces for Partial Differential Equation Control

Recent work has shown that reinforcement learning (RL) is a promising approach to control dynamical systems described by partial differential equations (PDE). This paper shows how to use RL to tackle more general PDE control problems that have continuous high-dimensional action spaces with spatial relationship among action dimensions. In particular, we propose the concept of action descriptors, which encode regularities among spatially-extended action dimensions and enable the agent to control high-dimensional action PDEs. We provide theoretical evidence suggesting that this approach can be more sample efficient compared to a conventional approach that treats each action dimension separately and does not explicitly exploit the spatial regularity of the action space. The action descriptor approach is then used within the deep deterministic policy gradient algorithm. Experiments on two PDE control problems, with up to 256-dimensional continuous actions, show the advantage of the proposed approach over the conventional one.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{enumitem}


%%%%%%%% Distribution definitions %%%%%%%%%%%%%%%

\newcommand{\normal}{\mathcal{N}}
\newcommand{\given}{|}

%%%%%%%% Matrix/vector definitions %%%%%%%%%%%%%%%

\newcommand{\inlinevec}[2]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1\\#2\end{smallmatrix}\Bigr]}}
\newcommand{\inlinemat}[4]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1 \ \ #2 \\#3 \ \ #4\\\end{smallmatrix}\Bigr]}}
\newcommand{\mathvec}[2]{\left[\begin{array}{c}#1\\#2\end{array} \right] }

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}
%\newcommand{\makevector}[1]{{\mathbf #1}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\eye}{\mathbf{I}}

%%%%%%%% Simple math functions %%%%%%%%%%%%%%%
\newcommand{\inv}{{\raisebox{.2ex}{$\scriptscriptstyle-1$}}}
\newcommand{\invt}{{\raisebox{.2ex}{$\scriptscriptstyle-\top$}}}
\newcommand{\pinv}{{\raisebox{.2ex}{$\scriptscriptstyle\dagger$}}}
\newcommand{\transpose}{{\raisebox{.2ex}{$\scriptscriptstyle\top$}}}
%\newcommand{\pinv}{\dagger}
\newcommand{\sgrad}{\partial}
\newcommand{\sign}[1]{\mathrm{sign}(#1)}
\newcommand{\posdef}{\succeq}
\newcommand{\e}{{\textrm{e-}}}
\newcommand{\Dom}{{\textrm{Dom}}}
\newcommand{\smallinv}[1]{{#1}^{\scalebox{0.5}[0.5]{\( - 1\)}}}

%%%%%%%% Norm definitions %%%%%%%%%%%%%%%
\newcommand{\frob}[1]{\left\| #1 \right\|_F}
\newcommand{\frobsq}[1]{\left\| #1 \right\|_F^2}
\newcommand{\frobsqtr}[1]{\text{tr}\left(#1'#1\right)}
\newcommand{\sqnorm}[1]{\Big\|  #1 \Big\|_{2}}
\newcommand{\spnorm}[1]{\left\|  #1 \right\|_{sp}}
\newcommand{\tracenorm}[1]{\left\|  #1 \right\|_{tr}}
\newcommand{\twonorm}[1]{\left\|  #1 \right\|_2}
\newcommand{\twoone}[1]{\left\|  #1 \right\|_{2,1}}
\newcommand{\bregman}[3]{D_{#1}(#2 \; || \: #3)}

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % RR numbers
\newcommand{\RRbar}{\overline{\RR}} % RR numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

% Set of [0, infty]
\newcommand{\RRpos}{{\RR^+}}

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\eigs}{\mathop{\mathrm{eigs}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nulls}{\mathop{\mathrm{null}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\spec}{\mathop{\mathrm{sp}}}
\newcommand{\sspan}{{\textrm{span}}}
\newcommand{\svd}{\mathop{\mathrm{svd}}}
\newcommand{\te}{\mathop{\mathrm{te}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\DeclareMathOperator\arctanh{arctanh}
%\newcommand{\ln}{\mathop{\mathrm{ln}}}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\set}[2]{\{#1 \ | \ #2\}}
\newcommand{\subfigurespace}[1]{ % Reasonable value = 0.1
\begin{minipage}[b]{#1\textwidth}
 \textbf{ }
 \end{minipage}}
 \newcommand{\figspace}{\begin{minipage}[b]{0.1\textwidth} \textbf{ } \end{minipage}}
\newcommand{\unaryminus}{\scalebox{0.75}[1.0]{\( - \)}}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}


%%%%%%%% Text definitions %%%%%%%%%%%%%%%

\newcommand{\apriori}{{\emph{a priori}}}
\newcommand{\emphdef}[1]{\textbf{#1}}
\newcommand{\introword}[1]{\textbf{\emph{#1}}}
\newcommand{\emphstart}[1]{\textbf{#1}}
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\subheader}[1]{
\vspace{8pt}
\noindent
{\large\bfseries #1}}

%%%%%%%% Examples of Stock standard definitions %%%%%%%%%%%%%%%
% This is just here as a reference for naming convention

%\newcommand{\xb}{\mathbf{x}}
%\newcommand{\xbtil}{\tilde{\xb}}
%\newcommand{\xtil}{\tilde{x}}
%\newcommand{\xhat}{\hat{x}}
%\newcommand{\xbhat}{\hat{\xb}}
%\newcommand{\Xtil}{\tilde{X}}
%\newcommand{\xbar}{\bar{x}}
%\newcommand{\xbbar}{\bar{\xb}}
%\newcommand{\Xb}{\mathbf{X}}
%\newcommand{\Xbtil}{\tilde{\Xb}}
%\newcommand{\Xbar}{\bar{X}}
%\newcommand{\Xbbar}{\bar{\Xb}}
%\newcommand{\Xhat}{\hat{X}}
%\newcommand{\Xbhat}{\hat{\Xb}}
%\newcommand{\Xcal}{\mathcal{X}}
%\newcommand{\Xtilde}{\widetilde{X}}
%\newcommand{\xvec}{\vec{x}}
%\newcommand{\Xvec}{\vec{X}}
%\newcommand{\xvecbar}{\bar{\vec{x}}}
%\newcommand{\xvechat}{\hat{\vec{x}}}
%\newcommand{\valhat}{\hat{\val}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\newcommand{\eproof}{$\null\hfill\blacksquare$}
%\ifx\proof\undefined
% \newenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\renewenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
%\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

% If end proof with align, then can add a negative space to bring up proof box
\newcommand{\palignbox}{\par \vspace{-0.8cm}}

\newif\ifsamenumbers

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\ifsamenumbers
\newtheorem{lemma}[theorem]{Lemma}
\else
\newtheorem{lemma}{Lemma}
\fi
\fi

\ifx\proposition\undefined
\ifsamenumbers
\newtheorem{proposition}[theorem]{Proposition}
\else
\newtheorem{proposition}{Proposition}
\fi
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\ifsamenumbers
\newtheorem{corollary}[theorem]{Corollary}
\else
\newtheorem{corollary}{Corollary}
\fi
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\ifsamenumbers
\newtheorem{conjecture}[theorem]{Conjecture}
\else
\newtheorem{conjecture}{Conjecture}
\fi
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\ifsamenumbers
\newtheorem{claim}[theorem]{Claim}
\else
\newtheorem{claim}{Claim}
\fi
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\myintertext}[1]{\end{enumerate} #1\begin{enumerate}[resume]}
\newenvironment{cenumerate}{%
\vspace{10pt}
\noindent{\Large\bfseries Contributions:}
\begin{enumerate}[label={\textbf{Contribution \arabic*.}\ },leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
}
{\end{enumerate}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}
\newcommand{\pca}{\text{\sc pca}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\meansmall}[1]{\mathop{\EE}[#1]}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


==> HDARL-PolicyGradient.tex <==
%%!TEX root = HDARL.tex


Policy gradient methods attempt to optimize some performance measure $J(\pi_\theta)$ of a policy, for example, the expected sum of rewards over a trajectory. The fundamental result makes this possible is the policy gradient theorem \cite{sutton2000pgfa}, which states that the gradient can be easily computed by establishing the connection between gradient of performance measure and gradient of (stochastic) policy. Mathemtaically, let $Q^{\pi_\theta}(\state, a)$ be the state action value under policy $\pi_\theta$ parameterized by $\theta$, stationary distribution is $d_{\pi_\theta}(\state), \forall \state \in \States$, then 
\begin{align*}
J(\pi_\theta) &= \int_\States d_{\pi_\theta}(\state) \int_{\Actions}^{} \pi_\theta (a | \state) Q^{\pi_\theta}(\state, a) da d\state \\
\nabla_\theta J(\pi_\theta) &= \int_\States d_{\pi_\theta}(\state) \int_{\Actions}^{} \nabla_\theta \pi_\theta (a | \state) Q^{\pi_\theta}(\state, a) da d\state \\
&= \int_\States d_{\pi_\theta}(\state) \int_{\Actions}^{} \pi_\theta (a | \state) \nabla_\theta \log \pi_\theta (a | \state) Q^{\pi_\theta}(\state, a) da d\state \\
&= \EE{\nabla_\theta \log \pi_\theta (a | X) Q^{\pi_\theta}(X, a) | X \sim d_{\pi_\theta}(x)}
\end{align*}

When dealing with continuous actions, the common way is letting the policy function output the mean of an action given current state and execute a sampled action after adding certain stochasticity (i.e. model the action is from the Gaussian distribution using the policy output as the mean). And hence the above $\pi_\theta (a | \state)$ is the action density function given a state. 

A popular policy gradient method is the actor-critic architecture, which can speed up the learning process. It uses an additional function to parameterize the state-action values, which serves as a critic for the actor (policy) function. In high dimensional or continuous state domains, we use function approximators (i.e. neural network) to generalize the critic. Below we introduce a competitive algorithm in various domains. 

\subsection{Deterministic policy gradient (DPG)}

Recent work about DPG \cite{lillicrap2016} develops the deterministic policy gradient theorem, and empircally showed that the algorithm can work well across various large physical control tasks. In this paper, we use our approach in the deep DPG algorithm as an example to perform experiments on multiple domains. To review the algorithm, we define the following notations. Given some state $\state$ and action $a$, let $\mu(\state; \actorparam)$ be actor network parameterized by $\actorparam$, $Q(\state, \action; \criticparam)$ be cirtic network parameterized by $\criticparam$. The $\criticparam$ is updated by using Q-learning formulae, while the $\actorparam$ is updated by using the gradient $\nabla_aQ(\state,a; \criticparam)|_{a=\mu(\state; \actorparam)} \nabla_\actorparam \mu(\state; \actorparam)$ derived through chain rule. It has been proved that $\nabla_a Q(\state,a; \criticparam)|_{a=\mu(\state; \actorparam)} \nabla_\actorparam \mu(\state; \actorparam)$ is the deterministic policy gradient \cite{silverlever2014} $\nabla_\theta J_\theta(\pi_\theta)$, where $\nabla_a Q(\state,a; \criticparam)|_{a=\mu(\state; \actorparam)}$ is the Jacobian matrix generated by taking gradient of each action component with respect to the actor network parameters. The DPG algorithm uses actor-critic architecture, solving the off-policy issue through Q learning update, hence it can easily allow any exploration stochasticity added to the action.

==> HDARL-PriorWork.tex <==
%%!TEX root = HDARL.tex

\newcommand{\xdim}{d}

In this section, we propose how to formulate a PDE control problem as a Markov decision process (MDP). We first provide a PDE control example, and then discuss how this could be viewed as a Markov decision process. We highlight that the key difference to previous approaches to formulating PDE control is that we consider infinite-dimensional actions, and exploit action regularities. 

%
%The most recent relevant work about using reinforcement learning algorithms to deal with PDE control problems is from \cite{FarahmandNabiNikovski2017} which attempts to solve a temperature control problem by modeling the underlying temperature change as a time-varying convection-diffusion PDE. In order to use reinforcement learning to solve the problem, it formulated the PDE as a Markov Decision Process (MDP), in which the action is defined in such a way that the boundary temperature can be controlled. The proposed algorithm, called deep Q-fitted iteration, utilizes convolutional layers to capture input state's regularities and is trained by setting a invariant targets of a batch of samples, which achieves same effect of using a separate target neural network. An earlier work \cite{FarahmandNabiGroverNikovski2016} takes another approach by using a reproducing kernel Hilbert space as the value function approximator. Both work focused on dealing with discrete action case and neither of them can be easily extended to high dimensional continuous action PDE control, where instead of regarding the action as changing the boundary values, we model an action as the source term in the PDE. 
%
%Below we give a short review of reinforcement learning setting and how high dimensional action PDE control can be formulated as a markov decision process. In a typical reinforcement learning control setting, we model the interaction between an agent and its environment as a Markov decision process $(\States, \Actions, \PKernel, \RKernel, \gamma)$, where $\States \subseteq \Real^d$ denotes state space, $\Actions \subseteq  \Real^k$ denotes the action space, and $\PKernel: \States \times \Actions \times \States \rightarrow [0, 1]$ encodes the transition probabilities and $\gamma$ is the discount rate. On each discrete time step $t = 1,2,3,...$, the agent selects an action according to some policy $\pi$ and the environment responds by transitioning into a new state $x_{t+1}$ sampled according to $\PKernel (x_ | x_t, a_t)$, and then the agent receives a scalar reward $r_{t+1} \eqdef \RKernel(\state_t, \action_t, \state_{t+1})$. $\gamma$ is the discount rate applied to the reward. 
%
%PDE control problems, we use the convection diffusion equation as an example. 
%
PDE control problems characterize a dynamical system using partial different equations. An example of such a set of equations is the convection diffusion equation
\begin{equation}
\frac{\partial T(z, t)}{\partial t}  = \nabla \cdot \frac{1}{P_e} \nabla T - \nabla \cdot (vT) + S(z, t)
\end{equation}
where $S(z, t)$ is the is the source or sink at a specific location $z$ and time $t$; $T(z, t)$ is the temperature function at $z$ and $t$; $\nabla \cdot$ is the divergence measuring the difference between a sink and source in the vector field; $\frac{1}{P_e}$ is a diffusivity constant; and $v$ is the velocity field which is a function of location and time $v = v(z, t)$.  This PDE describes how the temperature changes at each location. 
These equations can be influenced or controlled through an action function, $a(z,t)$, which influences the source term. Hence we further decompose the source term $S(z, t) = S^o(z, t) + a(z ,t)$.  
%The airflow is the same as the previous paper, two fans on two sides of the room respectively, a fan will be trigged if the sum of absolute value of the air conditioners' temperature on the corresponding half area of the room is greater some threshold. 

To relate this to the reinforcement learning setting, consider the state space $\States$, action space  $\Actions$ and transition dynamics $\PKernel$.
Typically, these spaces are assumed to be finite-dimensional, such as for continuous state where $\States$ is a subset of a $\xdim$-dimensional Euclidean space, $\mathbb{R}^\xdim$.  Here, however, the state and action are infinite dimensional vectors (functions) $\state_t = T(\cdot, t), \action_t = S(\cdot, t)$, where the two function's inputs are the same: $z \in \ZZ$. The state $\state_t$ is an infinite-dimensional vector, because it could be evaluated at all possible spatial locations, $z \in \ZZ$, where $\ZZ$ is a continuous space. The current state corresponds to the current temperature all all locations, and the action can increase or decrease the source value at each location. The next state is a random variable $X_{t+1} \sim \PKernel (\state | \state_t, \action_t)$. In the deterministic case, $\PKernel (\state | \state_t, \action_t) = \delta (\state - f(\state_t, \action_t))$, where $\delta(\cdot)$ is the Dirac's delta function and $\state_{t+1} = f(\state_t, \action_t) = T(\cdot, t) + \alpha_T \frac{\partial T(\cdot, t)}{\partial t}$, where $\alpha_T$ is some stepsize describing how fast the dynamic system changes. Finally, the reward function is designed based on the intuition that we want to save energy meanwhile also want to keep the room temperature at a comfortable level. 
\begin{align*}
&r(\state_t, \action_t, \state_{t+1}) = \\
& - \int_{z \in \ZZ}^{} I ({|T(z, t+1) - T^\ast(z, t+1)| > \epsilon}) dz \\
&- cost(\action_t)
\end{align*}
where $I(\cdot)$ is an indicator function, $T^\ast(\cdot)$ is a predefined function describing the most comfortable temperature, and high-cost actions are penalized with $cost(\cdot)$. 

Reinforcement learning algorithms, however, are not designed to learn with infinite-dimensional states and actions. 
We can overcome this problem, however, by exploiting the spatial regularities in the problem, and beyond PDEs, exploiting general regularities
between states and actions. We provide more intuition for these regularities, and then introduce MDPs with action-descriptors, a general subclass of infinite-dimensional MDPs, that provide a feasible approach to solving these infinite-dimensional problems. 

\subsection{Regularities in PDEs}

In reinforcement learning setting, we never directly deal with infinite dimensional matrices. In fact, the temperature can be measured at only certain finite locations in the room. We assume that we have totally $d$ measurement locations and $k$ controllable air conditioners uniformly distributed on the floor of the room, resulting in $\States = \Real^d, \Actions = \Real^k$. Note that $\ZZ$ becomes $d$ points specifying those measurement locations on the floor. We then design $cost(a) = \frac{||a||}{k}$. We will provide more details about those settings in experimental section and appendix. 

